An extreme thermal cycling reliability test of ATLAS ITk Strips barrel modules

At the end of Run 3 of the Large Hadron Collider (LHC), the accelerator complex will be upgraded to the High-Luminosity LHC (HL-LHC) in order to increase the total amount of data provided to its experiments. To cope with the increased rates of data, radiation, and pileup, the ATLAS detector will undergo a substantial upgrade, including a replacement of the Inner Detector with a future Inner Tracker, called the ITk. The ITk will be composed of pixel and strip sub-detectors, where the strips portion will be composed of 17,888 silicon strip detector modules. During the HL-LHC running period, the ITk will be cooled and warmed a number of times from about ${-35}^\circ$C to room temperature as part of the operational cycle, including warm-ups during yearly shutdowns. To ensure ITk Strips modules are functional after these expected temperature changes, and to ensure modules are mechanically robust, each module must undergo ten thermal cycles and pass a set of electrical and mechanical criteria before it is placed on a local support structure. This paper describes the thermal cycling Quality Control (QC) procedure, and results from the barrel pre-production phase (about 5% of the production volume). Additionally, in order to assess the headroom of the nominal QC procedure of 10 cycles and to ensure modules don't begin failing soon after, four representative ITk Strips barrel modules were thermally cycled 100 times - this study is also described.

==> Extra/Unused_and_extra_Material.tex <==
% \subsection{BNL-PPB2-MLS-211}
% \label{subsec:BNL-PPB2-MLS-211}

% \begin{figure}[htbp]
% \centering
% \includegraphics[width=1.0\textwidth]{Images/Trends/bnl211trends.pdf}
% \caption{\textcolor{red}{Propose BNL-PPB2-MLS-211 trend plot from Erik}\label{fig:fig}}
% \label{fig:bnl-211-trends}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\textwidth]{Images/Emulating_Lifetime_Of_TC/HV/BNL-211-April24_25.pdf}
%     \caption{\ew{Experimenting with HV current plots, placeholder data }}
%     \label{fig:enter-label}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\textwidth]{Images/Emulating_Lifetime_Of_TC/HV/BNL-211-May22_23.pdf}
%     \caption{\ew{Experimenting with HV current plots, placeholder data }}
%     \label{fig:enter-label}
% \end{figure}


% \ew{BNL-PPB2-MLS-211 sees an increase in the drawn PS and AMAC high voltage currents, before the Xth cold test. After this cycle, the power supply's current compliance limit was reached at a sensor of bias of -385 V (what does the IV look like before cycling?) indicating an early breakdown in the sensor. For the remainder of the cycles, the sensor bias was lowered to -250 V while it continued to be tested with readout electronics that were still nominal. 


% The trends in noise and gain can be seen in Fig. \ref{fig:bnl-211-trends}, where no trending in behavior is seen in the tests between the lowering of the sensor bias until cycle X, where  there was a complete electrical failure, where the output noise and gain significantly deviates from the original value. 

% The input noise in the first and last cold test is shown in Fig. \ref{fig:bnl-211-noise}. After the electrical failure, the input noise has increased across the whole module, with peaks near the powerboard on the under-side strips. 
% }

% \begin{figure}[htbp]%
%     \setcounter{subfigure}{0}
%     \centering
%     \subfloat[A]{\includegraphics[width=.475\textwidth]{Images/Emulating_Lifetime_Of_TC/Before_And_After_InputNoise/BNL_PPB2_MLS_211_Comparison_Input_noise_0_series.pdf}}%
%     \hfill
%     \subfloat[B]{\includegraphics[width=.475\textwidth]{Images/Emulating_Lifetime_Of_TC/Before_And_After_InputNoise/BNL_PPB2_MLS_211_Comparison_Input_noise_1_series.pdf}}%
%     \caption{Input noise in BNL-PPB-MLS-211 in the first and last cold test. Separately showing a) the under-side strip and b) the away-side strips.  }
%     \label{fig:bnl-211-noise}%
% \end{figure}  

% IV curve after cycling:

% \begin{figure}[htbp]%
%     \setcounter{subfigure}{0}
%     \centering
%     \subfloat[A]{\includegraphics[width=.475\textwidth]{Images/Emulating_Lifetime_Of_TC/IVs/BNL-PPB2-MLS-211_20.0degC_IVCurve.pdf}}%
%     \hfill
%     \subfloat[B]{\includegraphics[width=.475\textwidth]{Images/Emulating_Lifetime_Of_TC/IVs/BNL-PPB2-MLS-211_bypass_AMAC_20.0degC_IVCurve.pdf}}%
%     \caption{Caption \label{fig:fig}}%
% \end{figure}  


% \subsection{Summary}
% \label{sec:results}

% \begin{itemize}
%     \item BNL-PPB2-MLS-210 high current and very high noise towards end, roughly 95th cycle or so.
%     \item BNL-PPB2-MLS-211 early breakdown
%     \item SCIPP-PPB\_LS-016 loss of LV current draw during electrical testing. 
%     \item SCIPP-PPB\_LS-019 least unstable behavior among the four modules.
%     \item Ratio of noise values between first and final cycles.
% \end{itemize}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.6\textwidth]{Images/Extreme_Thermal_Cycling/LV/SCIPP-PPB_LS-016_LV.png}
%     \caption{Caption}
%     \label{fig:SCIPP-PPB_LS-016_LV}
% \end{figure}

% \ew{Module summary: 
% \begin{itemize}
%     \item Survives electrically
%     \item After warm cycle 57 (in my indexing) there is an LV problem. Module seems ok, but it starts to intermittently give strange tests, often with unusual Vt50, so seems like configuration issues. See LV in Fig. \ref{fig:SCIPP-PPB_LS-016_LV}. Abe: After cycling, we found the connector of the DisplayCable was a bit bent. Perhaps this led to imperfect electrical contact, and indeed may have messed with the configuration.
%     \item Two noise peaks, clearly seen in both input and output noise appear during the cycling. Not with very high amplitudes though.
% \end{itemize}
% }

==> Sections/Acknowledgments.tex <==
% \acknowledgments

% This work has been supported by the National Natural Science Foundation of China (No. 11961141014)
